Beyond Code Generation: LLM-supported Exploration of the Program Design Space

In this work, we explore explicit Large Language Model (LLM)-powered support for the iterative design of computer programs. Program design, like other design activity, is characterized by navigating a space of alternative problem formulations and associated solutions in an iterative fashion. LLMs are potentially powerful tools in helping this exploration; however, by default, code-generation LLMs deliver code that represents a particular point solution. This obscures the larger space of possible alternatives, many of which might be preferable to the LLM's default interpretation and its generated code. We contribute an IDE that supports program design through generating and showing new ways to frame problems alongside alternative solutions, tracking design decisions, and identifying implicit decisions made by either the programmer or the LLM. In a user study, we find that with our IDE, users combine and parallelize design phases to explore a broader design space -- but also struggle to keep up with LLM-originated changes to code and other information overload. These findings suggest a core challenge for future IDEs that support program design through higher-level instructions given to LLM-based agents: carefully managing attention and deciding what information agents should surface to program designers and when.

==> macros.tex <==
% for tool names
\usepackage{xspace}
\newcommand{\tool}[0]{\textsc{Pail}\xspace}
\newcommand{\baseAgent}[0]{\textsc{ConversationAgent}\xspace}
\newcommand{\designAgent}[0]{\textsc{DesignAgent}\xspace}
\newcommand{\reflectionAgent}[0]{\textsc{ReflectionsAgent}\xspace}

% for lozenges
\usepackage{tikz}
\newcommand\mybox[2][]{\tikz[overlay]\node[fill=blue!20,inner sep=2pt, anchor=text, rectangle, rounded corners=1mm,#1] {#2\xspace};\phantom{ #2}}

\newcommand{\loz}[2][blue]{~\mybox[fill=#1!20]{\textsc{#2}}}
\newcommand{\tryButton}[0]{ \loz[blue]{Try}\xspace}
\newcommand{\revertButton}[0]{ \loz[orange]{Revert}\xspace}

\newcommand{\dqSec}[0]{ \loz[green]{DQs}\xspace}
\newcommand{\crSec}[0]{ \loz[red]{Reqs}\xspace}
\newcommand{\idSec}[0]{ \loz[purple]{Decs}\xspace}
\newcommand{\uaSec}[0]{ \loz[teal]{UAbs}\xspace}

\newcommand{\dg}[1]{\loz[darkgreen]{DG{#1}}}

% For tables
\usepackage{multirow}
\usepackage{makecell}

%% Always center and bold face column headers
\newcommand\colH[1]{\multicolumn{1}{c}{\textbf{#1}}}
\newcommand\colHR[1]{\multicolumn{1}{r}{\textbf{#1}}}
\newcommand\colsH[2]{\multicolumn{#1}{c}{\textbf{#2}}}

% For quotes
\newcommand{\shortquote}[1]{``\emph{#1}''}


% For writing
%% ACTIVE
% \newcommand{\keyIdea}[1]{\textcolor{blue}{#1}}

%% INACTIVE
\newcommand{\keyIdea}[1]{#1}

% For commenting

%% ACTIVE
\newcommand{\jd}[1]{{\color{red} JD: #1 }}
\newcommand{\eunice}[1]{{\color{green} Eunice: #1 }}
\newcommand{\michael}[1]{{\color{orange} Michael: #1 }}
\newcommand{\qian}[1]{{\color{purple} Qian: #1 }}
\newcommand{\bjoern}[1]{{\color{purple} Bjoern: #1 }}

%% INACTIVE
% \newcommand{\jd}[1]{}
% \newcommand{\eunice}[1]{}
% \newcommand{\michael}[1]{}
% \newcommand{\qian}[1]{}
% \newcommand{\bjoern}[1]{}


%%% FOR REVISION
\definecolor{darkgreen}{rgb}{0,0.5,0}

%%% === R&R redline version === %%%
% \newcommand{\edits}[1]{{\color{darkgreen}#1\normalfont}}
% \usepackage[normalem]{ulem}
% \usepackage{soul}
% \newcommand{\deletes}[1]{\textcolor{red}{\sout{#1}}}

%%% === R&R clean version === %%%
\newcommand{\edits}[1]{#1}
\newcommand{\deletes}[1]{}


==> paper_ack.tex <==
The authors would like to thank the many individuals who supported this work, including: Chetan Goenka and Keira Swei, undergraduate researchers supported in their contributions to this work through Berkeley's Engineering Design Scholars summer program; Timothy J. Aveni, Shm Garanganao Almeda, James Smith, and Shreya Shankar, for many fruitful discussions on the concepts underlying this work, as well as feedback on drafts of this paper; our study participants, who graciously gave their time and feedback to this effort; and our anonymous reviewers, whose thoughtful comments shaped many revisions here.

J.D. Zamfirescu-Pereira was partially supported by a Google PhD Fellowship. Qian Yang's effort was supported in part by the AI2050 Early Career Fellowship program at Schmidt Sciences.
This material is also based upon work supported by the National Science Foundation under Grant No. 2313078.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.

==> tab_participants.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2} 
\begin{tabular}{c|c|c|c|c|c|c} 
\toprule
\textbf{ID} & \textbf{Age} & \textbf{Parent?} & \textbf{Professional Background} & \textbf{Design Experience} & \textbf{Programming Experience} & \textbf{LLM Use}
  \\ 
\hline
P1 & 40s & Yes & Design Researcher & Professional & Professional & Infrequent \\
P2 & 20s & - & HCI Graduate Student & Professional & Professional & Frequent \\
P3 & 30s & - & HCI Researcher & Amateur & Professional & Frequent \\
P4 & 30s & - & Software Eng Manager & None & Professional & Infrequent  \\
P5 & 50s & - & Software Eng Manager & Professional & Professional & Moderate \\
P6 & 60s & - & Film \& Media Artist & Professional & Amateur & Frequent \\
P7 & 20s & - & HCI Graduate Student & Professional & Amateur & Infrequent \\
P8 & 40s & Yes & Filmmaker \& Academic & Limited & Limited & Infrequent \\
P9 & 50s & - & Sound Artist \& Lecturer & Professional & Amateur & Infrequent \\
P10 & 60s & - & Software Engineer & Amateur & Professional & Moderate \\
P11 & 50s & Yes & Software Engineer & Limited & Professional & Moderate \\
% P12 & 40s & Product Manager & Minimal & Has heard of \llms \\
\bottomrule

\end{tabular}
\captionsetup{width=0.95\linewidth}
\vspace{0.2cm}
    \caption{Study participants.}
    \label{tab:participants}
    %\vspace{-3em}
\end{table*}
